Mad Max: Affine Spline Insights into Deep Learning

We build a rigorous bridge between deep networks (DNs) and approximation theory via spline functions and operators. Our key result is that a large class of DNs can be written as a composition of max-affine spline operators (MASOs), which provide a powerful portal through which to view and analyze their inner workings. For instance, conditioned on the input signal, the output of a MASO DN can be written as a simple affine transformation of the input. This implies that a DN constructs a set of signal-dependent, class-specific templates against which the signal is compared via a simple inner product; we explore the links to the classical theory of optimal classification via matched filters and the effects of data memorization. Going further, we propose a simple penalty term that can be added to the cost function of any DN learning algorithm to force the templates to be orthogonal with each other; this leads to significantly improved classification performance and reduced overfitting with no change to the DN architecture. The spline partition of the input signal space that is implicitly induced by a MASO directly links DNs to the theory of vector quantization (VQ) and $K$-means clustering, which opens up new geometric avenue to study how DNs organize signals in a hierarchical fashion. To validate the utility of the VQ interpretation, we develop and validate a new distance metric for signals and images that quantifies the difference between their VQ encodings. (This paper is a significantly expanded version of A Spline Theory of Deep Learning from ICML 2018.)

==> abstract.tex <==
{We build a rigorous bridge between deep networks (DNs) and approximation theory via spline functions and operators.
%
Our key result is that a large class of DNs can be written as a composition of max-affine spline operators (MASOs), which provide a powerful portal through which to view and analyze their inner workings.
% using tools from approximation theory and functional analysis.
%The MASO viewpoint leads to a number of key findings and interpretations.
%
For instance, conditioned on the input signal, the output of a MASO DN can be written as a simple affine transformation of the input.
%
This implies that a DN constructs a set of signal-dependent, class-specific templates against which the signal is compared via a simple inner product; we explore the links to the classical theory of optimal classification via matched filters and the effects of data memorization.
%
Going further, we propose a simple penalty term that can be added to the cost function of any DN learning algorithm to force the templates to be orthogonal with each other; this leads to significantly improved classification performance and reduced overfitting with no change to the DN architecture. 
%
The spline partition of the input signal space that is implicitly induced by a MASO directly links DNs to the theory of vector quantization (VQ) and $K$-means clustering, which opens up new geometric avenue to study how DNs organize signals in a hierarchical fashion.
%
To validate the utility of the VQ interpretation, we develop and validate a new distance metric for signals and images that quantifies the difference between their VQ encodings. 
 (This paper is a significantly expanded version of a paper with the same title that will appear at ICML 2018.)}
 {Splines, Deep Learning, Vector Quantization}

==> softmaso.tex <==
\section{Entropy Regularization for Soft-MASO}
\label{sec:inference}
\green{STORY : 1) define inference problem for MASO 2) see its link with reconstruction error, tie with bilinear coding 3) define entropy regularized inference problem leading to soft-MASO}

During the forward pass, the MASOs of the DN perform the maximization task as described in \ref{eq:maxDN1},\ref{eq:maxDN2}. This maximization inheriting from the max-affine spline property can be casted into an optimization problem over the style representation $[t^{(\ell)}(\bx)]_{k,.}$ by constraining it to belong to the space $\bigtriangleup_R = \{t \in [0,1]^R:\sum_{r=1}^R [t]_r=1\}$.
As such we can now rewrite the max-affine spline internal maximization over the parameters indices $r$ as a maximization process over the style encoding $[t^{(\ell)}(\bx)]_{k,.}$ as follows.
\begin{theorem}
\label{thm:tmaxi}
The max-affine spline maximization which produces its output can be rewritten in term of a constrained style vector as 
\begin{align}
    [\bz^{(\ell)}(\bx)]_k&=\max_{r \in \{1,\dots,R^{(\ell)}_k\}} \langle \bA^{(\ell)}[k,r],\bz^{(\ell-1)}(\bx) \rangle+\bB^{(\ell)}[k,r]\nonumber \\
    &=\max_{t \in \bigtriangleup_{R^{(\ell)}_k} }\sum_{r=1}^{R^{(\ell)}_k} t_r (\langle \bA^{(\ell)}[k,r],\bz^{(\ell-1)}(\bx) \rangle+\bB^{(\ell)}[k,r]),
    \label{eq:tmasoeq}
\end{align}
with $[t^{(\ell)}(\bx)]_{k,.}=\argmax_{t \in \bigtriangleup_{R^{(\ell)}_k} }\sum_{r=1}^{R^{(\ell)}_k} [t]_r (\langle \bA^{(\ell)}[k,r],\bz^{(\ell-1)}(\bx) \rangle+\bB^{(\ell)}[k,r])$ corresponding to the style vector from \ref{eq:tmaso}.
\end{theorem}



Another interesting extension lies in the possible regularization of $[t^{(\ell)}(\bx)]_{k,.}$ during this inference process. In particular, we will consider adding an Entropy regularization over $[t^{(\ell)}(\bx)]_{k,.}$. We will demonstrate that with such regularization, the new optimum style vector corresponds to a smooth (as opposed to 1-hot) style encoding which in turn leads to a MASO nonlinearity equal to the \textit{optimal} heuristically found nonlinearity of \cite{ramachandran2017searching} we denote as soft-MASO.

In order to enforce a smoother style representation, synonym of uncertainty, we introduce a regularization term in the maximization problem of (\ref{eq:tmasoeq}). Specifically, given the simplex space in which $[t^{(\ell)}(\bx)]_k$ is already constrained to belong to, one can directly apply Entropy regularization. Let first remind the Shannon Entropy \cite{shannon1959mathematical} as
\begin{equation}
    H(t)=-\sum_{r=1}^R [t]_r\log([t]_r),
\end{equation}
for any density distribution $t \in \bigtriangleup_R$. Based on this we can now develop the soft-MASO as follows.


\begin{theorem}
\label{thm:entropy_reg}
The Entropy regularized maximization problem \richb{what problem where?  you have to point to equation number or theorem numbers}\randall{the one below ?}
with convex weighting parameter $\beta$ leads to a soft style vector leading to a soft-MASO of the form of a  gated activation: 
\begin{align}
    \bz^{(\ell)}(\bx)_k&=\max_{t \in \bigtriangleup_{R^{(\ell)}_k} }\beta \underbrace{\sum_{r=1}^{R^{(\ell)}_k} [t]_r (\langle \bA^{(\ell)}[k,r],\bz^{(\ell-1)}(\bx) \rangle+\bB[k,r])}_{\text{Original Problem}}\nonumber\\
    &+(1-\beta) \underbrace{H(t)}_{\text{H-Regularization}}\nonumber \\
    &=\sum_{r=1}^{R^{(\ell)}_k}\left[\frac{e^{\frac{\beta}{1-\beta}(\langle \bA^{(\ell)}[k,r],\bz^{(\ell-1)}(\bx) \rangle+\bB^{(\ell)}[k,r])}}{\sum_{j=1}^{R^{(\ell)}_k} e^{\frac{\beta}{1-\beta}(\langle \bA^{(\ell)}[k,j],\bz^{(\ell-1)}(\bx) \rangle+\bB^{(\ell)}[k,j]) }}\right.\nonumber\\
    &\left.\times (\langle \bA^{(\ell)}[k,r],\bz^{(\ell-1)}(\bx) \rangle+\bB^{(\ell)}[k,r])\right].
\end{align}
Soft-MASO is thus a convex combination of the linear mapping with those convex coefficients being proportional to the linear mapping outputs, found via use of a softmax nonlinearity. It is clear that $\beta \rightarrow 1$ leads to standard inference of Thm. \ref{thm:tmaxi} while $\beta \rightarrow 0 $ leads to a linear mapping of the form 
\begin{align}
    [\bz^{(\ell)}(\bx)]_k&=\frac{1}{R}\sum_{r=1}^R \langle \bA^{(\ell)}[k,r],\bz^{(\ell-1)}(\bx) \rangle+\bB^{(\ell)}[k,r]).
\end{align}
Proof in \ref{sec:proof_entropy_reg}.
\end{theorem}
\iffalse
\begin{proof}
We denote $c_r=\langle a_r,x\rangle+b_r$, we then obtain the constrained optimization problem solve via KKT and Lagrange multipliers in this order has we have strong duality we solve as follows
\begin{align*}
    \mathcal{L}(s)=&\beta \sum_r c_rs_r+(1-\beta)H(y)\\
    \frac{\partial \mathcal{L}}{\partial s_p}=&\beta c_p-(1-\beta)\log(s_p)-(1-\beta)+\gamma\\
    \frac{\partial \mathcal{L}}{\partial \gamma}=&\sum_r s_r-1\\
    \frac{\partial \mathcal{L}}{\partial s_p}=0 \implies & s_p=e^{\frac{\beta}{1-\beta}-1+\frac{\beta}{1-\beta}c_p}\\
    \frac{\partial \mathcal{L}}{\partial \gamma}=0 \implies & \gamma = (1-\beta)\left( -\log(\sum_r e^{\frac{\beta}{1-\beta}c_r})+1 \right)\\
    \implies & s_p=\frac{e^{\frac{\beta}{1-\beta}c_p}}{\sum_r e^{\frac{\beta}{1-\beta}c_r}},
\end{align*}
By a straightforward second order computation one can see that this corresponds to a local maximum. Being the only critical point, it corresponds to a global maximum.
\end{proof}
\fi
%Note that while being out of scope in this report, the optimization problem above is identical to the one of entropy regularization optimal transport and should be further studied.
Now that soft-MASO has been derived, we see how it corresponds to nonlinearities found to be \textit{empirically optimal} in diverse settings. Let first start with the soft-MASO based on the ReLU nonlinearity.

\begin{cor}
With ReLU MASO, we obtain the optimal nonlinearity empirically found in 
\cite{ramachandran2017searching} by setting $\beta=0.5$. In fact applying directly the above theorem with the ReLU parameters and entropy regularization, one obtains
\begin{align}
    [\bz^{(\ell)}(\bx)&]_k=\frac{\langle e^{\bA^{(\ell)}[k,2],\bz^{(\ell-1)(\bx)}\rangle+\bB^{(\ell)}[k,2]}}{1+e^{\langle \bA^{(\ell)}[k,2],\bz^{(\ell-1)}(\bx)\rangle+\bB^{(\ell)}[k,2]}}\nonumber \\
    &\times (\langle \bA^{(\ell)}[k,2],\bz^{(\ell-1)}(\bx)\rangle+\bB^{(\ell)}[k,2])\nonumber \\
    =&\sigma_{sigmoid}(\langle \bA^{(\ell)}[k,2],\bz^{(\ell-1)}(\bx)\rangle+\bB^{(\ell)}[k,2])\nonumber \\
    &(\langle \bA^{(\ell)}[k,2],\bz^{(\ell-1)}(\bx)\rangle+\bB^{(\ell)}[k,2])\nonumber \\
    =&\sigma_{sigmoid}(\langle [\bC^{(\ell)}]_{k,.},\bz^{(\ell-1)}(\bx)\rangle+[\bb_{\bC}^{(\ell)}]_{k})\nonumber \\
    &\times (\langle [\bC^{(\ell)}]_{k,.},\bz^{(\ell-1)}(\bx)\rangle+[\bb_{\bC}^{(\ell)}]_{k})
\end{align}
with $1$ for the first region exponential as $e^{\langle \bA^{(\ell)}[k,2],\bz^{(\ell-1)}(\bx)\rangle+\bB^{(\ell)}[k,1]}=e^0=1$ and the last line demonstrating the case where ReLU activation and convolution was the internal layer configuration for illustrative purposes.
\end{cor}


This last corollary demonstrates how for ReLU soft-MASO one obtains the standard gated activation function empirically found in \cite{ramachandran2017searching} which corresponds to applying the affine transform followed by gating the output by an Hadamard product between this affine transform output and this affine transform output fed into a sigmoid activation function.
We now perform the same for max-pooling for which we obtain softmax-pooling.
\begin{cor}
For max-pooling MASO, setting $\beta=0.5$ corresponds to the softmax pooling formulated in \cite{boureau2010theoretical}
\end{cor}

This derivation of soft-MASO with controllable parameter $\beta$ allows to have a differentiable, simple parameter leading to a layer interpolated between being a standard MASO or a fully linear one. Incorporation of such parameter optimization into current DN would lead to more stable results and would allow undesirable layers to be set to linear thus being less detrimental for the whole mapping. Note that behavior control of DN mappings was for example proposed in \cite{gulcehre2016mollifying} where during learning a DN is initialized with linear behaviors for faster learning.




